EasyGenNet: An Efficient Framework for Audio-Driven Gesture Video Generation Based on Diffusion Model

Audio-driven cospeech video generation typically involves two stages: speech-to-gesture and gesture-to-video. While significant advances have been made in speech-to-gesture generation, synthesizing natural expressions and gestures remains challenging in gesture-to-video systems. In order to improve the generation effect, previous works adopted complex input and training strategies and required a large amount of data sets for pre-training, which brought inconvenience to practical applications. We propose a simple one-stage training method and a temporal inference method based on a diffusion model to synthesize realistic and continuous gesture videos without the need for additional training of temporal modules.The entire model makes use of existing pre-trained weights, and only a few thousand frames of data are needed for each character at a time to complete fine-tuning. Built upon the video generator, we introduce a new audio-to-video pipeline to synthesize co-speech videos, using 2D human skeleton as the intermediate motion representation. Our experiments show that our method outperforms existing GAN-based and diffusion-based methods.

==> figures/5_qualitive_audio2video.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.8\linewidth]{images/audio2vid3}
        \vspace{-10pt}
    \caption{Video sequences generated by our method. We visualized the results of continuous video frames generated for two characters. Our method synthesizes accurate appearances, clear hands, and temporally coherent results.}
    \label{fig:5_qualitive_audio2video} 
        \vspace{-10pt}
\end{figure}

==> macros/common.tex <==

% figures and sections
\newcommand{\reffig}[1]{Figure~\ref{fig:#1}}
\newcommand{\refsec}[1]{Section~\ref{sec:#1}}
\newcommand{\refapp}[1]{Appendix~\ref{sec:#1}}
\newcommand{\reftbl}[1]{Table~\ref{tab:#1}}
\newcommand{\refalg}[1]{Algorithm~\ref{alg:#1}}
\newcommand{\refline}[1]{Line~\ref{line:#1}}
\newcommand{\shortrefsec}[1]{\S~\ref{sec:#1}}
\newcommand{\refeq}[1]{Equation~\ref{eq:#1}}
\newcommand{\refeqshort}[1]{(\ref{eq:#1})}
\newcommand{\shortrefeq}[1]{\ref{eq:#1}}
\newcommand{\lblfig}[1]{\label{fig:#1}}
\newcommand{\lblsec}[1]{\label{sec:#1}}
\newcommand{\lbleq}[1]{\label{eq:#1}}
\newcommand{\lbltbl}[1]{\label{tab:#1}}
\newcommand{\lblalg}[1]{\label{alg:#1}}
\newcommand{\lblline}[1]{\label{line:#1}}
% \newcommand{\shortcite}[1]{\cite{#1}}
% \newcommand{\deps}{\bs{\epsilon}_\theta}
% \newcommand{\depsh}{\bs{\hat{\epsilon}}_\theta}
% \newcommand{\prompt}[1]{``\emph{#1}"}
% \newcommand{\afterfigure}{\vspace{-1em}}

% \definecolor{MyDarkBlue}{rgb}{0,0.08,1}
\newcommand{\camera}[1]{#1}

% \newcommand{\myparagraph}[1]{\vspace{-3pt}\paragraph{#1}}
% \newcommand{\myparagraph}[1]{\paragraph{#1}}
\newcommand{\myparagraph}[1]{\vspace{5pt} \noindent \textbf{#1} \ }
% \newcommand{\ours}{DreamLoop\xspace}
% \newcommand{\ours}{\xspace}
\newcommand{\feature}{\bs{f}_{t}\xspace}

\newcommand{\website}{\href{https://text2cinemagraph.github.io/website/}{\textit{website}}\xspace}
%     \bs{z}^*_{style(t-1)}, \{\bs{A}^i_{style(t)}\} = \bs{\hat{\epsilon}_\theta}(\bs{z}^*_{style(t)}, \bs{P}_{style}, t)
% \end{equation}
% Then for generation of \nat, we inject the $\bs{A}^i_t$ and $\phi^{4}_t$, during the reverse denoising process of generation of \nat,
% \begin{equation}
%     \bs{z}^*_{real(t-1)} = \bs{\hat{\epsilon}_\theta}(\bs{z}^*_{real(t)}, \bs{P}_{real}, t\;;\; \phi^{4}_{style(t)}, \{\bs{A}^i_{style(t)}\})
% \end{equation}


% \newcommand{}

\newcommand{\bs}[1]{{\boldsymbol{#1}}}
% \newcommand{\pixel}{p\xspace} % pixel coordinates
% \newcommand{\art}{\bs{x}\xspace} % aristic image 
% \newcommand{\nat}{\hat{\bs{x}}\xspace} % noisy image 
% \newcommand{\artt}{\bs{x}_t\xspace} % noisy artistic image at timestemp t
% \newcommand{\natt}{\hat{\bs{x}}_t\xspace}  % noisy natural image at timestemp t
% \newcommand{\arttminus}{\bs{x}_{t-1}\xspace}  % noisy artistic image at timestemp t-1
% \newcommand{\nattminus}{\hat{\bs{x}}_{t-1}\xspace}  % noisy natural image at timestemp t-1
% \newcommand{\atten}{\bs{A}_t\xspace}  % artistic image's self-attention map 
% \newcommand{\attenavg}{\bs{\overline{A}}\xspace}  % artistic image's self-attention map 
% \newcommand{\artmask}{\bs{M}\xspace}   % artistic image's mask
% \newcommand{\natmask}{\hat{\bs{M}}\xspace}  % natural image's mask 
% \newcommand{\artflow}{\bs{F}\xspace}  % artistic image's flow
% \newcommand{\natflow}{\hat{\bs{F}}\xspace} % natural images' flow

% \newcommand{\at}{\bs{c}\xspace}   % artistic image's prompt
% \newcommand{\nt}{\hat{\bs{c}}\xspace} % natural image's prompt 
% \newcommand{\gf}{\bs{G}_{flow}\xspace}
% \newcommand{\gv}{\bs{G}_{frame}\xspace}

\newcommand{\A}{\bs{A}\xspace}  %audio
\newcommand{\M}{\bs{M}\xspace}  %untextured mesh
% \newcommand{\M_hat}{\bs{\hat{M}}\xspace}  %textured mesh
\newcommand{\N}{\bs{N}\xspace}  %normal
\newcommand{\D}{\bs{D}\xspace}  %depth
\newcommand{\V}{\bs{V}\xspace}  %video
\newcommand{\C}{\bs{C}\xspace}  %conditioning
\newcommand{\ren}{\bs{I}\xspace}  %conditioning
\newcommand{\gf}{\bs{G}_{\text{frame}}\xspace}     %frame generator
\newcommand{\cam}{\bs{P}\xspace}  %conditioning
\newcommand{\uv}{\bs{U}_{\text{tex}}\xspace}  %conditioning

% OLD
% \newcommand{\pixel}{p\xspace}
% \newcommand{\art}{\bs{x}_{style}\xspace}
% \newcommand{\nat}{\bs{x}_{real}\xspace}
% \newcommand{\artt}{\bs{x}_{style, t}\xspace}
% \newcommand{\natt}{\bs{x}_{real, t}\xspace}
% \newcommand{\arttminus}{\bs{x}_{style, t-1}\xspace}
% \newcommand{\nattminus}{\bs{x}_{real, t-1}\xspace}
% \newcommand{\at}{\bs{c}_{style}\xspace}
% \newcommand{\nt}{\bs{c}_{real}\xspace}
% \newcommand{\gf}{\bs{G}_{flow}\xspace}
% \newcommand{\gv}{\bs{G}_{frame}\xspace}
% \newcommand{\prompt}{c\xspace}
% \renewcommand{\empty}{\varnothing}  % {\emptyset}

% \newcommand{\latent}{{z}}

% \makeatletter
% \def\adl@drawiv#1#2#3{%
%         \hskip.5\tabcolsep
%         \xleaders#3{#2.5\@tempdimb #1{1}#2.5\@tempdimb}%
%                 #2\z@ plus1fil minus1fil\relax
%         \hskip.5\tabcolsep}
% \newcommand{\cdashlinelr}[1]{%
%   \noalign{\vskip\aboverulesep
%            \global\let\@dashdrawstore\adl@draw
%            \global\let\adl@draw\adl@drawiv}
%   \cdashline{#1}
%   \noalign{\global\let\adl@draw\@dashdrawstore
%            \vskip\belowrulesep}}
% \makeatother
